Optimal Strategies of Blotto Games: Beyond Convexity

The Colonel Blotto game, first introduced by Borel in 1921, is a well-studied game theory classic. Two colonels each have a pool of troops that they divide simultaneously among a set of battlefields. The winner of each battlefield is the colonel who puts more troops in it and the overall utility of each colonel is the sum of weights of the battlefields that s/he wins. Over the past century, the Colonel Blotto game has found applications in many different forms of competition from advertisements to politics to sports. Two main objectives have been proposed for this game in the literature: (i) maximizing the guaranteed expected payoff, and (ii) maximizing the probability of obtaining a minimum payoff $u$. The former corresponds to the conventional utility maximization and the latter concerns scenarios such as elections where the candidates' goal is to maximize the probability of getting at least half of the votes (rather than the expected number of votes). In this paper, we consider both of these objectives and show how it is possible to obtain (almost) optimal solutions that have few strategies in their support. One of the main technical challenges in obtaining bounded support strategies for the Colonel Blotto game is that the solution space becomes non-convex. This prevents us from using convex programming techniques in finding optimal strategies which are essentially the main tools that are used in the literature. However, we show through a set of structural results that the solution space can, interestingly, be partitioned into polynomially many disjoint convex polytopes that can be considered independently. Coupled with a number of other combinatorial observations, this leads to polynomial time approximation schemes for both of the aforementioned objectives.

==> cg2.tex <==
\section{Randomizing over More than Two Pure Strategies}\label{section:nonuniformc>2}
We extend the results of Sections~\ref{sec:continuous} and~\ref{sec:integral} to more than two pure strategies. More precisely, the problem that we study in this section is the following: given that there exists a \maxmin{u}{p} strategy that randomizes over $c$ pure strategies, our goal is to approximate such a strategy in polynomial time. When $c=1$, we have only one pure strategy and we play that pure strategy with probability $1$. For the case of $c=2$, we play two pure strategies. In this case, we may play the first strategy with probability $q$ and the second strategy with probability $q' = 1-q$. An important observation here is that for the case of $c=2$, we can assume w.l.o.g. that $q = 1-q = 1/2$. To prove this, let us assume for the sake of contradiction that $q > 1/2 > q'$.  Thus, we play a strategy $\b{x}$ with probability $q$ and a strategy $\b{x}'$ with probability $q'$. Moreover, assume that our strategy is \maxmin{u}{p} for some $u, p > 0$. This means that against any best-response  $y$ of player 2 our strategy wins a utility of $u$ with probability at least $p$. Since $p$ is nonzero, then either $\b{x}$ or $\b{x}'$ wins a utility of at least $u$ against any strategy of player 2. Therefore, $p \geq \min\{q,q'\} = q'$ holds. In addition to this, if $p > q'$, it means that if $\b{x}$ guarantees a utility of $u$ against all pure strategies of player 2 and therefore player 1 could have played $\b{x}$ and win a utility of $u$ with probability $1$. Obviously, playing $\b{x}$ and $\b{x}'$ is not optimal since playing $\b{x}$ alone would give player 1 a better guarantee here. Also, in case $p = \min{q,q'} = q'$, the optimal way to randomized over $\b{x}$ and $\b{x}'$ is to play each of them with probability $1/2$ so that $p = 1/2$ is maximized.

However, when $c > 2$, an optimal \maxminc{u}{p}{c} strategy, does not necessarily play the pure strategies with equal probabilities! As an example, assume that $c = 3$ and player 1 plays three pure strategies $\b{x}$, $\b{x}'$, and $\b{x}''$ with the property that against any strategy of player 2, either $\b{x}$ gets a utility of at least $u$, or both $\b{x}'$ and $\b{x}''$ get a utility of at least $u$. In this case, the optimal way to randomize over $\b{x}, \b{x}',$ and $\b{x}''$ is to play $\b{x}$ with probability $1/2$ and play each of $\b{x}'$ and $\b{x}''$ with probability $1/4$ (or any combination that sums up to $1/2$).

\sbcomment{To be continued.}


==> multiplediscrete__mahsa_derakhshan_s_conflicted_copy_2018-03-16_.tex <==


\mdcomment{c-strategty}

\mdcomment{introduction of this section goes here}
\begin{theorem}
			Given that player 1 has a \maxminc{u}{p}{2} strategy, there exists a polynomial time algorithm that obtains a \maxminc{(1-\epsilon)u}{p}{2} strategy of player 1 for any arbitrarily small constant $\epsilon > 0$.
\end{theorem}

Given that the first player randomized over two pure strategies $\b{x}$ and  $\b{x}$, the second player's best response is a strategy that maximizes his payoff. That is, player 2 seeks to find a strategy $\b{y} \in \puresetb$ such that $\min(\utilityb{\b{x}}{\b{y}}, \utilityb{\b{x}}{\b{y}})$ is maximized.
Also, when player 1 randomizes over two pure strategies we assume that he cannot guarantee utility $u$ for himself, otherwise he would just play one pure strategy. Also, when a \maxminc{u}{p}{2} strategy is guaranteed, there are two pure strategies $\b{x}$,  $\b{x}$ of the first player where $\min(\utilityb{\b{x}}{\b{y}}, \utilityb{\b{x}}{\b{y}}) \geq $ for any $\b{y} \in \puresetb$. Therefore, we assume that in a \maxminc{u}{p}{2} strategy, $p = 0.5$.  Although, there exist polynomial time algorithms to find the best response of player 2, we still need more simpler algorithms to be able to use them for finding an optimal \maxminc{u/2}{p}{2} strategy for player 1. \mdcomment{clarify} To this end, we assume that the second player takes a simple greedy approach instead of solving the problem optimally. We first give an alternative formation of the best response problem in which the solution is represented by two binary vectors. We then relax the integrality condition of elements in the vectors and prove that, there is a fractional solution to this problem where the number of fractional elements in each vector is at most one. Using this characteristic of the problem we give a greedy algorithm for the best response problem and prove that if player 2 plays the strategy given by this algorithm, he losses at most $\wmax$ payoff compared to his best response strategy. Recall that $\wmax$ denotes the maximum weight of the battlefields.

To give an alternative formulation of the best response problem, we define a new problem in which any solution is represent  by two vectors of size $k$. Given strategies $\b{x}$ and $\b{x'}$ we first define vectors $\b{c}$ and $\b{c'}$. For any battlefield $i$, if $x_i \leq x'_i$ then $c_i := x_i$ and $c'_i := x'_i - x_i$. Otherwise,  $c'_i := x'_i$ and $c_i := x_i - x'_i$. Roughly speaking, when $x_i \leq x'_i$ holds, $c_i$ is the number of troops that player 2 needs to put in battlefield $i$ to win strategy $x$ in this battlefield and $c'_i$ is the number of troops that he should add to win both strategies. The solution to this problem is two vectors $\b{h}$ and $\b{h'}$ that maximizes $\min(\b{w}\b{h}, \b{w}\b{h'})$ subject to the following conditions.
\begin{enumerate}
\item For any $i\in [k]$, elements $h_i$ and $h'_i$ are binary variables. 
\item If $x_i \leq x'_i$, then $h'_i \leq h_i$ holds. Otherwise,  $h_i \leq h'_i$ holds.  \label{condition 2}
\item Also, $\b{c} \cdot \b{h} + \b{c'} \cdot \b{h'} \leq m$.  \label{condition 3}
 \end{enumerate}
 Given vectors $\b{h}$ and $\b{h'}$, the solution of this problem, one can find a strategy $\b{y}$ of player 2 where $ u=\b{w}\b{h}$ and $u'=\b{w}\b{h}$. (Recall that $u$ and $u'$ respectively denote the utility that strategy $\b{y}$ gets against strategies $\b{x}$ and $\b{x'}$.) We claim that if for any $i\in [k]$, player 2 puts $h_i\cdot c_i + h'_i \cdot c'_i$ troops in battlefield $i$, then $u \geq \b{w}\b{h}$ and $u' \geq \b{w}\b{h}$ hold. 
 Note that by condition \ref{condition 3}, he has enough troops to play this strategy.  Without loss of generality, assume that $x_i \leq x'_i$. Therefore by condition \ref{condition 2}, $h'_i \leq h_i$ holds. There are three possible cases. Either both $h'_i$ and $h_i$ are 0, both are equal to 1, or $h'_i = 0$ and $h_i=1$.  
If $h_i = h'_i = 0$, then $w_i \cdot h_i $ and $w'_i \cdot h'_i$ are both equal to zero. In the case of $h_i = 1$ and $h_i=0$, we have $h_i\cdot c_i + h'_i \cdot c'_i = x_i$. Therefore in battlefield $i$, player 2 gets utility $w_i$ against strategy $x_i$. Also, if $h_i = h'_i = 1$, the equality $h_i\cdot c_i + h'_i \cdot c'_i = x'_i$ holds, which means player 2 gets utility $w_i$ against both strategies in this battlefield.
 Thus, in all three cases, the utility that player 2 gets against strategies $\b{x}$ and $\b{x'}$ in battlefield $i$ is receptively at least $w_i \cdot h_i$ and at least $w'_i \cdot h'_i$. 
 
  Moreover, given any strategy $\b{y}$ of player 2, one can give two valid vectors \b{h} and \b{h'} such that $u = \b{w}\b{h}$ and $u' = \b{w}\b{h}$. Iff $y_i \geq x_i$, let $h_i := 1$. Also iff $y_i \geq x'_i$, we set $h'_i := 1$. Therefore,  $u = \b{w}\b{h}$ and $u' = \b{w}\b{h}$ hold. We also need to show that $\b{c\cdot h} + \b{c' \cdot h'} \leq m$. For this, it suffices to show $\b{c_i\cdot h_i} + \b{c_i' \cdot h_i'} \leq y_i$ for any $i\in [k]$. Without loss of generality, assume that $x_i \leq x'_i$. Thus, $c_i = x_i$ and $c'_i = x'_i - x_i$ hold. Note that we can assume that $y_i$ is either 0, $x_i$ or $x'_i$. In all these three cases,  $\b{c_i\cdot h_i} + \b{c_i' \cdot h_i'} \leq y_i$ holds therefore vectors \b{h} and \b{h'} satisfy the necessary conditions.

To sum up, for any solution of the defined problem which we denote by vectors $\b{h}$ and $\b{h'}$ there is a strategy of the opponent with payoff $\b{c} \cdot \b{h} + \b{c'} \cdot \b{h'}$. Also, for any \maxminc{u}{p}{2} strategy of player 2,  there are two vectors $\b{h}$ and $\b{h'}$  that satisfy the necessary conditions of the problem where $\min(\b{w}\b{h}, \b{w}\b{h'}) = u$ holds for them. Therefore, this formulation is indeed a valid formulation of the best response problem. 

\subsubsection{Fractional Strategy of The Opponent}
 
Any strategy of the player 2 can be represented by two vectors $\b{h}$ and $\b{h'}$. If we relax the integrality constraint of the strategies for player 2, elements of these vectors can be fractional numbers between 0 and 1. We call such a strategy a fractional strategy.
In this section, we give an algorithm to find the best fractional strategy of the opponent and prove that ....\mdcomment{integrality gap}


\begin{lemma}
If vectors $\b{h}$ and $\b{h'}$ represent a best fractional strategy of the opponent against any arbitrary 2-strategy of the first player, then $\b{w}\b{h} = \b{w}\b{h'}$ holds.
\end{lemma}
\begin{proof}

We use proof contradiction. We assume  that a  pair of $\b{h}$ and $\b{h'}$ are given and they do not satisfy $\b{w}\b{h} = \b{w}\b{h'}$. By modifying $\b{h}$ and $\b{h'}$ we give two new vectors $\b{\eta}$ and $\b{\eta'}$ such that they are a valid representation of second player's strategy and $\min(\b{w}\b{h}, \b{w}\b{h'}) < \min(\b{w}\b{\eta}, \b{w}\b{\eta'})$. This means that strategy denoted by vectors $\b{h}$ and $\b{h'}$ is not a best strategy of the opponent which is a contradiction.  
\mdcomment{Give $\b{\eta}$ and $\b{\eta'}$}
\end{proof}

\begin{lemma}
Algorithm~\ref{alg:2-fractional} gives the best fractional response  of the second player.
\end{lemma}

\begin{proof}
Proof of this lemma goes here.	
\end{proof}

\begin{algorithm}
	\caption{Best fractional strategy of the second player}
	\label{alg:2-fractional}
	\begin{algorithmic}[1]
		\Statex \textbf{Input:} strategies $\b{x}$ and $\b{x'}$ of the first player and vector $\b{w}$ which is the battlefields' weight vector.
		\Statex \textbf{Output:} a fractional strategy $\b{y} = (y_1, \ldots, y_k)$ of player 2.
		\State $\b{c}, \b{c'} \gets (0, \ldots, 0)$
		\For{$i \in [k]$}
			\If{$x_i \leq x'_i$} 
			\State $c_i := x_i$ and $c'_i := x'_i - x_i$
			\Else
			\State  $c'_i := x'_i$ and $c_i := x_i - x'_i$
			\EndIf
		\EndFor
		\State $a \gets \{arg: \}$
		\State \mdcomment{Algorithm goes here}
		\State \Return $\b{y}$
	\end{algorithmic}	
\end{algorithm}


\begin{lemma}
Let strategy $\b{y} = (y_1, \ldots, y_k)$ denote the fractional strategy of player 2 that is obtained from Algorithm~\ref{alg:2-fractional}. There are at most two indices $i, j\in [k]$ where $h_i$ or $h'_i$ is a fractional number.   
\end{lemma}

\begin{proof}
WE use proof by contradiction. We first assume that for either $\b{h}$ or $\b{h'}$ and prove it for one of them. (The same proof holds for the other one.) Assume, there are two indices $i, j \in $ where $h_i$ and $h_j$ are both fractional. Note that the algorithm is sequential and at each time, in just increases one of the elements in \b{h}. We prove that either one of $h_j$ and $h_i$ that increases first, becomes integral before we start changing the other one.
\mdcomment{complete the proof.}    
\end{proof}

\begin{algorithm}
	\caption{\maxminc{u/2}{p}{2} strategy of player 1}
	\label{alg:2-integral}
	\begin{algorithmic}[1]
		\Statex \textbf{Input:} vector $\b{w}$ which is the battlefields' weight vector.
		\Statex \textbf{Output:} $\b{x}$, a \maxminc{u/2}{p}{2} strategy of the first player.
		\State $S_1 = {i : i\in []}$
		\State S'_1
		\State S_2
		\State \mdcomment{Algorithm goes here}
		\State \Return $\b{x}$
	\end{algorithmic}	
\end{algorithm}

\begin{theorem}
Given that there exists a \maxminc{u}{p}{2} strategy for the first player, Algorithm \ref{alg:2-integral} gives a \maxminc{u/2}{p}{2} strategy of this player in polynomial time.
\end{theorem}










